FORGE: Feasible Online Reduced-Order Reference Generation and Whole-Body Execution for Agile Humanoid Locomotion

This paper presents a two-stage learning framework for versatile and agile humanoid locomotion that couples online reduced-order model (ROM) reference generation with whole-body tracking control. In the first stage, we train a command-conditioned whole-body reference generator using single rigid body dynamics combined with full humanoid kinematics. In the second stage, the frozen ROM policy is rolled out online to generate references for training a whole-body tracking policy on the full-order dynamics model. Learning a kino-dynamically consistent reference generator in the simplified ROM space enables us to generate references over a broad command space and over multiple locomotion strategies using a single unified framework. We demonstrate the approach on a Unitree G1 humanoid robot, achieving longitudinal velocities from -2.0 m/s to 2.8 m/s, lateral velocities up to +-1.0 m/s, angular velocities up to +-3.0 rad/s, one-legged hopping, and continuous transitions across the commands, all using one unified reference policy and one whole-body tracking policy.

==> fom_reward_table.tex <==
% Requires \usepackage{booktabs} and \usepackage{amsmath,amssymb}
\begin{table}[t]
\centering
\caption{Reward terms used for FOM (whole-body tracking) training.}
\label{tab:fom_rewards}
\footnotesize
\setlength{\tabcolsep}{4pt}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{@{}lcc@{}}
\toprule
\textbf{Reward Term} & \textbf{Expression} & \textbf{Weight} \\
\midrule
\textbf{Motion tracking} & & \\
Body orientation      & $\exp(\lVert(q_{b},q_{b}^{d}\lVert^2/\sigma^2)$ & $1.0$ \\
Body pos./vel.        & $\exp(\lVert e_{b}\rVert^2/\sigma^2)$ & $1.0$ \\

Root position         & $\exp(-\lVert p_{\mathrm{r}}-p_{\mathrm{r}}^{d}\rVert^2/\sigma^2)$ & $0.5$ \\
Root orientation      & $\exp(-\angle(q_{\mathrm{r}},q_{\mathrm{r}}^{d})^2/\sigma^2)$ & $0.5$ \\
\midrule
\textbf{Regularization} & & \\
Action-rate           & $\lVert a_t - a_{t-1}\rVert^2$ & $-0.1$ \\
Joint limit           & $\lVert(\underline{q}-q_t)^{+} + (q_t-\bar{q})^{+}\rVert^2$ & $-10.0$ \\
Self-collision        & $\#\{f_{\mathrm{c}}>f_{\mathrm{thr}}\}$ & $-10.0$ \\
Feet slide (lin.)     & $\textstyle\sum_{\mathrm{ft}}\lVert v_{\mathrm{ft},xy}\rVert\,c_{\mathrm{ft}}$ & $-0.4$ \\
Feet slide (rot.)     & $\textstyle\sum_{\mathrm{ft}}\lvert\omega_{\mathrm{ft},z}\rvert\,c_{\mathrm{ft}}$ & $-0.1$ \\
\midrule
\textbf{ROM twist-command tracking} & & \\
Twist ($v_x,v_y,\omega_z$) & $\exp(-((\zeta-\zeta^{\mathrm{cmd}})/\sigma)^2)$ & $0.5$ \\
% \midrule
% \textbf{ROM contact matching} & & \\
% Contact-mode match    & $\pm 1\ (\text{match}/\text{mismatch})$ & $0.5$ \\
% Contact-mode streak   & $r_{\min}+(r_{\max}-r_{\min})\,k/k_{\max}$ & $0.5$ \\
\bottomrule
\end{tabular}%
}
\end{table}
